Structured Scaling of AI Discovery Across Diverse Scientific Domains

Scientific discovery often requires many cycles of proposing, testing, and refining candidate solutions. Language models can increasingly participate in these loops, but simply generating more attempts does not ensure progress: parallel searches may duplicate one another and iterative refinement may become trapped in poor directions. The central challenge is therefore not only to scale AI-driven discovery, but to structure that scaling so that evaluation signals compound over time. Here we introduce SimpleTES (Simple Test-time Evaluation-driven Scaling), a framework that focuses on the structured scaling of AI discovery loops, organizing evaluator queries across independent trajectories, iterative refinement, local candidate selection, and the selective reuse of evaluated histories. Drawing on structural features of scientific communities, SimpleTES uses a single open-source GPT-OSS model to establish new state-of-the-art solutions across 28 open-ended problems in diverse scientific domains ranging from quantum physics and astronomy to biology, AI, and mathematics. These include a 24.5% reduction in quantum circuit compilation overhead, up to 23% lower propulsive cost for deep-space trajectories, a 2.17x faster lasso-path solver, an 8.5% lower-error whole-brain neural-activity predictor, the fastest reported TriMul kernel, and new mathematical constructions beyond prior human or AI records. We further post-train the model for long-horizon discovery by assigning each attempt the final outcome of the trajectory it helped produce. This improves performance on both training and held-out mathematics problems, further advancing the frontier. Together, these results establish structured scaling as a general mechanism for advancing AI scientific discovery.

==> sections/main_method.tex <==
\subsection*{Methods}
\label{sec:framework}

\subsubsection*{The evaluation-driven discovery loop}
\label{sec:tes}

Recent studies on test-time scaling (TTS) improve model performance by increasing test-time computation, such as using more reasoning tokens~\citep{muennighoff-etal-2025-s1}, multi-turn sampling~\citep{inoue2025wider}, or agentic workflows with tool use and search~\citep{chakraborty2025feedback,chen2025tumix}. 
For scientific discovery, cycles of trial-and-error guided by external feedback are the foundation of breakthroughs.
This motivates a central question: whether and how the evaluation-driven loop can be effectively scaled up.
This form of scaling focuses on problems where an evaluation surrogate is both \emph{necessary} and \emph{available}, ruling out problems whose evaluation is purely subjective or currently intractable. 

The evaluation-driven loop can be formalized as follows.
Given a problem instruction $x_0 \in \mathcal X$ in the text space, we aim to discover a solution $y \in \mathcal{Y}$ that maximizes a true underlying objective. 
In real-world scientific discovery, this true objective is rarely directly accessible, so the discovery process relies on an explicit, queryable surrogate evaluator $V\colon \mathcal{Y} \to \mathbb R \times \mathcal M$.
For a candidate solution $y$, the evaluator returns $V(y)=(r,m)$, where $r\in\mathbb R$ is a scalar score, and $m\in\mathcal M$ contains auxiliary feedback or metadata, such as verifier messages, error traces, or other task-specific information.
With access to this evaluator, the question can be stated precisely as: whether and how scaling the number of evaluation queries $N$ enables the discovery of a solution with a high score $r$, which is expected to also perform well under the true objective.

The discovery process is controlled by a policy $\pi$ equipped with a language model $G\colon \mathcal X \to \mathcal Y$\footnote{We fix $G$ to a single LLM, as we aim to study the scaling effect of evaluation queries. Nevertheless, it can be replaced by more complex designs, including model ensembles~\citep{novikov2025alphaevolve,lange2025shinkaevolve}, tool-using agentic workflows~\citep{yao2023react,shinn2023reflexion,baek-etal-2025-researchagent,schmidgall2025agentlab,chakraborty2025feedback,chen2025tumix}, and trainable test-time-adapted models~\citep{yuksekgonul2026learning,wang2025thetaevolve,zweiger2025selfadapting}.}. 
Specifically, $\pi$ is initialized from a solution $y_0$, which may be a naive baseline or an existing strong solution, with $(r_0,m_0)=V(y_0)$ being the initial score and feedback.
Whenever the policy needs to, it can create a new \emph{proposal} $x_n$, which may include instructions, historical solutions and feedback, statistics from past attempts, and any other information needed by $G$ to generate the next solution $y_n$. 
Once generated, $y_n$ is evaluated by $V$, and the resulting node $(y_n,r_n,m_n)\in\mathcal Y\times\mathbb R\times\mathcal M$ is returned to the policy for constructing future proposals. 
This process continues until the evaluator-query budget $N$ is exhausted, and the highest-scoring solution is returned.

Notice that practical policies can be, and often are, asynchronous: multiple generation or evaluation jobs may be launched simultaneously, results may arrive out of order, and the policy may act before all earlier jobs have completed. 
This makes the space of possible policies extremely broad, ranging from simple refinement loops to complex evolutionary or agentic systems. 
A comprehensive review of existing designs of $\pi$ can be found in Supplementary~\ref{sec:related:existing_tte}. 
While these methods leverage evaluators in different ways, they often treat feedback as one component of a broader search procedure, rather than \emph{explicitly} studying the scaling effect of the evaluation-driven loop itself. 
Evaluation-driven scaling instead asks what happens when the feedback-driven discovery loop is scaled up through more evaluator queries, rather than only scaling generation-side computation such as reasoning length, sampling count, or agent turns.

\paragraph{Remark on $V$.}
The assumption of an evaluator surrogate does not guarantee its perfect alignment with the true objective. 
Depending on the nature of the problem, the fidelity of the evaluator $V$ exists on a spectrum.
It can be the \emph{exact metric} we care about, such as a mathematical verifier ensuring the strict correctness of a construction, or a program counting the exact number of circles packed in a given square;
It can be an \emph{empirical estimation} of the metric, such as timing a GPU kernel on a subset of test cases to approximate its overall execution speed. 
It can also be a \emph{heuristic proxy}, such as a regression loss evaluated on a limited training dataset, which potentially correlates with the true generalization capability.
This inherent discrepancy between the surrogate evaluator and the true objective can lead to various forms of reward hacking~\citep{amodei2016concrete,gao2023rewardoveroptimization,pang2023rewardgaming} or overfitting~\citep{cawley2010overfitting,recht2019imagenetv2}, challenges that we systematically analyze below.

\subsubsection*{Scaling the loop with $(C, L, K, \Phi)$}
\label{sec:method:rewrite}

The key question is how evaluator queries should be used effectively. A naive best-of-$N$ policy spends the entire budget on independently sampled candidates, failing to use evaluator feedback to guide later attempts. A sequential refinement policy, on the other hand, uses feedback to improve later candidates, but commits the search to a single trajectory and can become trapped by early choices. 
Recent approaches demonstrate the power of iterative discovery systems that combine generation, evaluation, and refinement. 
Building on this evidence, this section asks a fundamental design question: how should evaluator queries be organized to use feedback most effectively? 

We introduce \method, a simple algorithmic framework for scaling the evaluation-driven discovery loop at test time. 
The key idea is to organize evaluator queries through a compact design space: $C$ independent trajectories provide global exploration, $L$ committed refinement steps accumulate feedback within each trajectory, $K$ local candidates are evaluated before each commitment, and $\Phi$ maps the committed history into the next proposal. 
We present the pseudo-code of \method in \Cref{alg:simpletes}, with its design space and analysis of each parameter specified below. We also discuss the theoretical insights for these parameter designs in Supplementary~\ref{app:CL_model}.

\begin{definition}
\label{def:hyper}
Given a problem instruction $x_0$, the hyper-parameter space (design space) of \Cref{alg:simpletes} is defined as
\begin{align}
    \mathcal H
    =
    \left\{
    (C,L,K,\Phi):
    C,L,K \in \mathbb N_+,\;
    \Phi \colon \mathrm{FinSet}(\mathcal Y\times \mathbb R\times \mathcal M) \to \mathcal X
    \right\}.
\end{align}
Here $C,L,K$ are the scaling dimensions of \method, $\Phi$ is a subroutine that creates new proposals $x$ based on historical information, and $\mathrm{FinSet}(\cdot)$ denotes the finite set of element instances. 
\end{definition}



\begin{algorithm}[t]
\caption{\method}
\label{alg:simpletes}
\begin{algorithmic}[1]
\Require instruction $x_0$, LLM $G$, evaluator $V$, initial solution $y_0$, parameter $(C,L,K,\Phi)\in\mathcal H$
\State $(r_0,m_0) \gets V(y_0)$, $S_0 \gets \{(y_0,r_0,m_0)\}$


\Function{Trajectory}{$S$}
    % \State $S \gets S_0$
    \For{$\ell=1,\dots,L$}
        % \State $S \gets \Call{LocalStep}{S}$
        \State $x \gets \Phi(S)$
        \State Generate $K$ candidates $\{y^{k}\}_{k=1}^{K} \sim G(x)$
        \State Evaluate each candidate: $(r^{k},m^{k}) \gets V(y^{k})$ for $k\in[K]$
        \State  $S \gets S \cup \{(y^{k^*},r^{k^*},m^{k^*})\}$ where $k^* = \mathop{\arg\max}_k r^{k}$ 
    \EndFor
    \State \Return $S$
\EndFunction

\State Run $C$ independent trajectories in parallel:
\begin{align*}
    S_1,\dots,S_C
    \gets
    \Call{Trajectory}{S_0},\dots,\Call{Trajectory}{S_0}.
\end{align*}
\State \Return $ \mathop{\arg\max}_{(y,r,m)\in \bigcup_{c=1}^{C} S_c} r$
\end{algorithmic}
\end{algorithm}

\paragraph{Terminology.}
A \emph{trajectory} is a sequence of $L$ refinement steps that starts from the initial node $(y_0, r_0, m_0)$ and accumulates evaluated nodes into a set $S$.
Each evaluated tuple $(y, r, m) \in S$ is called a \emph{node}, representing a solution along with its score and metadata.
The \emph{context construction} mapping $\Phi$ selects which historical nodes from $S$ to include in the next generation proposal $x = \Phi(S)$.
By default, \method allows each generation to condition on multiple historical nodes rather than only the immediate predecessor, enabling flexible recombination of successful patterns across the trajectory.


\paragraph{From sequential refinement to independent search.}
To understand the design choice of \method, we start with a simple, straightforward evaluation-driven scaling policy: \emph{sequential refinement}. Specifically, it generates a candidate, evaluates it, uses all historical feedback to generate a better one, and repeats. 
$\pi_\text{seq}$ corresponds to a special case in Definition~\ref{def:hyper} parameterized by $(1, L, 1, \Phi)$. 

Yet sequential refinement has a fundamental limitation. Open-ended problems require multidimensional coverage: a high-quality solution must simultaneously satisfy multiple criteria (correctness, efficiency, generality, etc.). But refinements are path-dependent: the direction of early attempts largely determines the space of subsequent improvements. This mismatch creates a ``Matthew Effect'' where early progress in one dimension attracts further refinement to that same dimension, starving alternatives and trapping the search around local optima.

To overcome this limitation, \method introduces a simple additional axis: global width $C$. Specifically, we run $C$ independent trajectories in parallel, each maintaining its own history and exploring possible directions for improvement separately. By enabling independent exploration, global width increases the chance that at least one trajectory starts from sufficiently diverse early attempts, allowing later refinements to compound into qualitatively better solutions.

For readers interested in a formal justification of this effect, we provide a mathematical model and theorem in Supplementary~\ref{app:CL_model}. Here, we empirically demonstrate the phenomenon by applying \method to two mathematical problems under different combinations of $C$ and $L$. As shown in \Cref{fig:method_ckl} (left), increasing $L$ initially improves performance but quickly saturates, consistent with the lock-in effect of a single refinement trajectory. In contrast, increasing $C$ provides a clear benefit by diversifying the committed histories explored under the same feedback-driven loop. This observation motivates global width as a key dimension of \method: before simply refining deeper, the policy should allocate evaluator queries to multiple independent trajectories.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{sections/figures/main_method/scaling_iso_budget.pdf}
    \caption{Performance of \method on two tasks (lower is better), autocorrelation inequalities (top) and Erd\H{o}s minimum overlap (bottom), under different global width $C$ (left) and local sample size $K$ (right). 
    Each curve shares the same query budget $N$, with deeper color corresponding to larger $N$. 
    The best configuration under the same budget is marked as ``star''. 
    We set $K=1$ (left) and $C=1$ (right) for simplicity.
    }
    \label{fig:method_ckl}
\end{figure}

\paragraph{From single samples to local batches.}
The introduction of $C$ is due to the nature of the problems, whereas the introduction of $K$, the local sample size, is due to the nature of the LLM. Even when a trajectory has identified a promising direction, a single call to the LLM can still produce a weak, noisy, or failed candidate. If such a candidate is immediately committed to the trajectory history, its errors may affect all subsequent refinements. This creates a local commitment risk at every refinement step.

Within each search trajectory, \method evaluates a batch of $K$ candidates for each proposal $x$ and adds only the highest-scoring one to the history. 
Under a fixed evaluator-query budget, introducing local sample size changes the allocation from $(C,L,1,\Phi)$ to approximately $(C,L/K,K,\Phi)$. 
The allocation between $L$ and $K$ creates a trade-off: a larger $K$ improves the quality of each committed step, but it reduces the number of refinement steps. 
A smaller local sample size $K$, on the other hand, makes the trajectory vulnerable to local generation noise that hurts future refinement.

As shown in \Cref{fig:method_ckl}, increasing $K$ from $1$ to a moderate value consistently improves performance, indicating that local greedy selection helps prevent weak samples from entering the trajectory history. However, when $K$ becomes too large and leaves only a small refinement depth $L$, the gains may saturate or even reverse, as the trajectory no longer has sufficient room to accumulate feedback over time. This motivates local sample size $K$ as another key dimension of \method: evaluator queries within a trajectory should balance the number of refinement steps with the reliability of each committed step.

\paragraph{From full history to compressed context.}
The discussion above focuses on how evaluator queries are allocated, which gives the three scaling dimensions $(C,L,K)$. 
This allocation view abstracts away another practical question: how the feedback accumulated along a trajectory is presented to the LLM. 
With an idealized LLM that has unlimited context, perfect attention, and the ability to extract all useful patterns from prior attempts, the policy could simply expose the entire committed history to it. 
Thus, $\Phi$ would not affect the allocation analysis above.

Real language models, however, are not ideal in this sense. 
The committed history of a trajectory can quickly become long, redundant, and noisy, containing solutions, scores, error messages, implementation details, and partial insights. 
Query construction is therefore a compression problem: the policy must convert the trajectory-local history into a generation proposal that fits the model's capacity while preserving the feedback most useful for the next refinement step. 
We formalize this as a mapping
\begin{align}
    \Phi:\mathrm{FinSet}(\mathcal Y\times\mathbb R\times\mathcal M)\to\mathcal X,
\end{align}
where each node $(y,r,m)$ contains a committed solution, its scalar score, and auxiliary metadata.
The design of $\Phi$ involves two sub-problems: \emph{history selection}, which decides which previous nodes should be exposed to the LLM, and \emph{prompt formatting}, which decides how these nodes should be presented. 
We discuss concrete instantiations below.

Together, \method provides a simple but effective abstraction for scaling evaluation-driven discovery loops. 
The design space $(C,L,K,\Phi)$ isolates the core dimensions of evaluation-driven scaling, including diverse exploration, feedback-driven refinement, and local greedy selection. 
This compact formulation gives a clean interface for studying scaling behavior while remaining practical across diverse scientific discovery problems.


% ===========================================================================
% END REWRITE
% ===========================================================================

\subsubsection*{Implementation details}
\label{sec:engineering}

This subsection specifies the implementation details of \method. 
Due to the independence of trajectories, we omit the trajectory index $c$ below.
Each trajectory is exposed to $\Phi$ only a finite set
\[
    S \subset \mathrm{FinSet} (\mathcal Y \times \mathbb R \times \mathcal M)
\]
of historical nodes $(y,r,m)$.
For clarity, we append necessary runtime metadata in $m$, including the proposal index for each node, the return index, and other lightweight bookkeeping information, such as which historical nodes were selected for context, how often each node has been selected, summarized failure patterns, and optional reflections.
This information is used in the definition of $\Phi$ and does not affect the algorithm design space.

\paragraph{Proposal created with historical nodes.}
The main role of $\Phi$ is to decide which previously explored experiences should be presented in a new proposal that can maximize the potential result of this new solution. 
This is achieved by deciding which nodes in $S$ should be included in $x=\Phi(S)$.
Our default approach is \textbf{RPUCG}, a graph-based extension of PUCT~\citep{alphazero2018,rosin2011multiarmed,silver2017mastering}.
Whenever a new solution is generated from a prompt that conditions on certain historical nodes, the implementation stores parent--child links among the corresponding nodes in $S$.
For a node indexed by $i$, let $\mathrm{Ch}(i)$ denote all nodes that have included node $i$ in their proposal (all nodes that are inspired by node $i$ up to now).
For each node, we maintain a propagated value
\begin{align}
\label{eq:propagate_score}
    U_i
    =
    \max\left(
        r_i,\;
        \gamma \max_{j\in \mathrm{Ch}(i)} U_j
    \right),
\end{align}
where $\gamma\in(0,1]$ is a discount factor.
The second term is ignored if $\mathrm{Ch}(i)$ is empty.

Intuitively, an experience is valuable either because (1) it already has a high evaluator score (so it should be able to inspire a similarly good solution), or (2) because its solution is inspiring and has led to strong descendants before. RPUCG balances the two reasons by the following formula:
\begin{align}
    \mathrm{RPUCG}(i)
    =
    U_i
    +
    \lambda \rho_i
    \frac{\sqrt{1+|S|}}{1+n_i},
\end{align}
where $\lambda$ controls exploration, $\rho_i$ is the relative prior of node $i$ based on its score percentile within the current $S$, and $n_i$ is the number of times $i$ has been previously included in the context of a proposal.

The first term favors nodes with strong propagated value, while the second is an exploration term that allows unexplored nodes (whose $n_i$ will be small) to be included.

To reduce redundancy, $\Phi$ selects historical nodes greedily according to $\mathrm{RPUCG}(i)$, while excluding the one-hop neighbors. We use multiple historical nodes for context construction, in contrast to sequential refinement and prior work~\citep{wang2025thetaevolve,yuksekgonul2026learning}, which condition on only a single node.
We use RPUCG as the default selector in the main paper; alternative selectors are described in Methods.

\paragraph{Prompt construction.}
After selecting historical nodes, $\Phi$ formats the next proposal $x$ for $G$.
Prompt design can substantially affect performance.
Prior systems such as~\citet{openevolve_github,wang2025thetaevolve,yuksekgonul2026learning} often use complex instructions with task-specific hints and expert-designed heuristics.
Such hints may improve performance, but they are difficult to curate and may not transfer across tasks.
In pilot experiments, removing these hints from \citet{wang2025thetaevolve} and using only a plain instruction caused a substantial performance drop, suggesting that prompt construction is itself an important design problem.

\method adopts a minimalist prompt strategy and moves most adaptation into the search procedure.
We avoid expert-crafted hints and manually specified error patterns.
Each prompt contains four types of information:
\begin{enumerate}
    \item the plain task instruction $x_0$;
    \item evaluation configurations, such as timeout and resource limits;
    \item selected historical nodes from $S$, including their scores, evaluator feedback $m$, and concise summaries of useful observations;
    \item optional automatically accumulated signals, such as repeated exceptions, timeout patterns, missing imports such as \texttt{numpy}, package information from \texttt{requirements.txt}, LLM-based reflections over committed winners, or validated artifacts that can serve as warm starts for constructive tasks. We ablate those design choices in Supplementary~\ref{sec:results:ablation}.
\end{enumerate}
These components add little direct human prior knowledge.
Instead, they are accumulated from experience during search and exposed through the same interface $x=\Phi(S)$.~\Cref{fig:prompt-comparison} compares the task-instruction prompts used by~\citet{wang2025thetaevolve} and \method.


\paragraph{Best-solution restart.}
One of the advantages of the \method is its design choice of initial solution $y_0$, which can be a naive solution or an existing strong result.
Therefore, a natural way to further scale up evaluation-driven loops is to start from solution obtained from previous \method runs.
We refer to this process as \emph{best-solution restart} strategy, where after a complete run finishes, we use the best discovered solution to initialize another identical run:
\[
    y_0 \leftarrow \arg\max_{(y,r,m)\in S} r .
\]
This will reset the trajectory histories and all implementation bookkeeping.
Notice that, empirically, we observe that most continual best-solution restarts will saturate; e.g., the second or third restart run could never have improved on the initial solution.
The saturation indicates that the underlying mechanism of best-solution restart remains underexplored, and therefore, we do not include this design in our main \method design space.
Throughout our experiments, we only run one additional best-solution restart unless otherwise specified.

\paragraph{Asynchronous execution.}
\Cref{alg:simpletes} describes the logical search process, while the runtime executes generation and evaluation asynchronously.
Each call to $\Phi(S)$ creates one logical local batch for one trajectory.
All $K$ candidates in the batch share the same proposal $x$, and the trajectory updates its $S$ only after the batch has finished.
Thus, the trajectory-level search semantics remain synchronized, even though generation and evaluation jobs may run concurrently and return out of order.

The implementation uses two worker pools, one for generation and one for evaluation, connected by bounded queues.
A local batch can be dispatched either as one $K$-sample generation request or as $K$ separate one-sample requests.
The two modes are semantically identical because they share the same proposal $x$ and are reduced by the same local best-of-$K$ commit rule.
The streamed mode improves overlap between generation and evaluation, while the batched mode reduces request overhead.

To prevent the runtime from drifting too far ahead of the policy state, we apply trajectory-level backpressure.
Each active trajectory may have only a bounded number of unresolved local batches.
With the default setting, a trajectory cannot launch a second local batch until the previous one has resolved, recovering strict trajectory synchronization.
Increasing this bound allows deeper pipelining.
The generation and evaluation queues are also physically bounded; when they are saturated, submission blocks rather than discarding work.
If no new proposal can be scheduled, the scheduler waits for either generation or evaluation progress.
The runtime does not evict already admitted generation or evaluation jobs; control is exerted at admission time.

\paragraph{Evaluation engineering.}
Executing thousands of untrusted LLM-generated programs requires strict isolation.
To reduce cost, we do not rely on cloud sandboxing services such as E2B~\citep{e2b_docs} or Daytona~\citep{daytona_sandboxes}; instead, each \method run is evaluated on a single compute node.
Each evaluation is executed in a fresh subprocess with process-group timeouts and memory limits, preventing infinite loops and resource leaks from affecting the broader system.
For more complex tasks, we additionally enforce container-level isolation through Docker, with networking disabled and temporary directories partitioned to prevent cross-run contamination.

To mitigate reward hacking, we implement independent score verification.
The system does not trust metrics reported by generated code.
Instead, an outer secure process independently recomputes final scores using isolated test data.
This separation between generated programs and evaluation data prevents models from exploiting hardcoded outputs or overfitting to exposed test cases, improving the reliability of the reported results.

\subsubsection*{Learning to scale the loop}
\label{sec:training}

The \method framework facilitates the generation of a massive amount of structured, high-quality search trajectories. 
All these histories are a natural form of supervision on how to learn from prior experience for future improvements, analogous to how a human researcher's experience accumulates into deeper scientific expertise. 
In this section, we propose a training paradigm that enables the model to systematically learn from trial-and-error experiences, thereby catalyzing subsequent scientific discoveries.

From the perspective of reinforcement learning~\citep{guo2025deepseek}, evaluation-driven scaling appears deceptively simple: every proposed solution candidate receives evaluator feedback, and one might therefore train the model to optimize each step according to its immediate reward. 
This training paradigm has been adopted by a few existing attempts~\citep{wang2025thetaevolve,yuksekgonul2026learning}.
However, this is not a short-horizon task in which each candidate should consistently achieve optimal scores; it is a long-horizon process in which early attempts may be valuable precisely because they expose failure modes, diversify the search, or create useful starting points for later refinement. 
A model trained only to prefer candidates with high instantaneous scores may therefore become overly conservative, missing the exploratory behaviors that attempt to jump out from the local optimum and enable later breakthroughs.
Consequently, the goal of the post-training process should shift from maximizing the quality of every intermediate solution to developing an awareness of the topology of evaluation-driven scaling: to learn how evaluator feedback should shape the trajectory of future attempts.

\paragraph{Trajectory-Level post-training.} In this paper, we post-train models at the trajectory level, rather than the instance level, to align the optimization objective with the long-horizon nature of evaluation scaling. Specifically, we conceptualize the entire trajectory as a ``rollout'' step, with each node--comprising a reasoning process and the proposed solution--representing an action. We deliberately bypass ALL intermediate rewards, and instead backpropagate the ultimate trajectory-level performance (i.e., the maximum score achieved across the entire history) to all constituent actions. By intentionally discarding myopic signals, this training objective becomes unbiased, ensuring that the model optimizes for the global breakthrough that aligns with the intention of scientific discovery, rather than local, potentially non-optimal, metrics.

The pseudo code of our post-training process is provided in \Cref{alg:irft}.
We apply standard RLVR optimization on a trajectory-level formulation that repeatedly executes the following steps: (1) performing \method inference to sample $\hat{C}$ independent trajectories with the current model $G$, (2) assigning scalar credits $w$ for each node based on trajectory-level scores, (3) optimizing the model with the following weighted objective:   
\begin{equation}
\label{eq:loss2}
    \mathcal{L} = -\mathbb{E}_{(x,\hat{y},w) \sim \mathcal{D}}\left[w\cdot \sum_{i=1}^{|\hat y| } \log \pi_\theta(\hat{y}_i \mid x, \hat{y}_{<i})\right],
\end{equation}

where $\mathcal{D}$ is the set of nodes obtained from the history, $x$ is the prompt, $\hat{y}$ is the response composed of reasoning contents and the solution, and $w$ is the assigned credit.


\begin{algorithm}[t]
\caption{Trajectory-Level Training for Evaluation-driven Scaling}
\label{alg:irft}
\begin{algorithmic}[1]
\Require problem set $\mathcal{P}$, initial model $G$, training iterations $T$, trajectory rollout size $\hat{C}$
\State $\mathcal{D}\gets \{\}$
\For{$t=1$ to $T$} 
    \For{$\mathrm{P}\in\mathcal{P}$}
    \State Run \method with $\hat{C}$ trajectories using model $G$ on $\mathrm {P}$, obtain $\{S_c\}_{c=1}^{\hat C}$
    \State Add all trajectories to dataset: $\mathcal{D}\gets \mathcal{D}\cup \{S_c\}_{c=1}^{\hat C}$

    \EndFor
    % \For {$(x,\hat{y})\in S$}
    \State Assign credit: $\mathcal W=\text{CreditAssignment}(\mathcal D)$
    \State Training $G$ with \Cref{eq:loss2}: $G\gets \text{Train}(G,\mathcal{D}, \mathcal W)$
    % \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

\paragraph{Credit assignment.} 
The fundamental challenge in trajectory-level post-training lies in the design of the credit assignment mechanism.
In terms of the concrete design choices, one may directly use the absolute terminate score similar to REINFORCE \cite{williams1992simple}, use a relative advantage similar to GRPO \cite{shao2024deepseekmath}, or even simply a binary reward similar to iterative rejection fine-tuning (IRFT) \cite{touvron2023llama}.
For simplicity, in this paper, we instantiate our training with the IRFT approach by assigning $w=1$ to trajectories with the top $R\%$ scores for each task, and $w=0$ to the remaining, which focuses the model’s learning capacity on high-quality trajectories. To improve data efficiency, we truncate and discard all nodes in a trajectory subsequent to the point where the maximal score first appears. This simple post-train approach turns out to be effective, as we will present in Supplementary~\ref{sec:analysis_train}. We leave studies on more data-efficient approaches to future work.

\paragraph{Engineering details.} 
In practice, we adopt additional engineering designs to ensure robust convergence and computational efficiency. First, due to the high cost of search sampling, we maintain a persistent replay buffer, i.e., instead of relying exclusively on on-policy rollouts that are discarded after a single training iteration, the historical nodes $\mathcal{D}$ are progressively accumulated and resampled, providing richer data for training. Besides, to avoid the cold-start problem, we set a larger rollout size $\hat{C}$ in the first iteration to populate the replay buffer with a diverse set of trajectories. Second, rather than maintaining a static threshold, we dynamically decrease the top-tier ratio $R$ as training continues. This adaptive mechanism prevents the volume of training data from scaling uncontrollably and ensures that the model is progressively trained on only the most elite trajectories as its performance improves.

==> sections/main_paper.tex <==
\begingroup

\subsection*{Introduction}
\label{sec:introduction}


% Scientific discovery rarely proceeds as a single act of reasoning; it is usually reached through repeated cycles in which researchers propose candidate solutions, test them against the world, and use the feedback to guide the next attempt~\citep{langley1987scientific}. 
% In astrodynamics, the intricate choreography of deep-space exploration is realized by proposing candidate gravity-assist trajectories, vetting them against rigorous orbital mechanics simulators, and refining maneuver timings to minimize propulsive costs~\citep{vasile2006MGA-diffculty,shen2026deepspacetrajectorydesign}.
% In quantum information science, variational algorithms, control protocols, and compilation strategies are improved through repeated hardware and simulator evaluations that expose errors, latency, and resource costs~\citep{cerezo2021variational, koch2022quantum,li2019tackling}. The high-performance GPU kernels behind today's AI models are tuned the same way, their tiling, memory layout, and instruction schedules refined iteratively against latency profiles~\citep{chetlur2014cudnn,narayanan2021efficient,dao2022flashattention}. Run in parallel by a community of researchers who build on one another's results, this \emph{propose--evaluate--refine} loop is how entire fields move forward.


% The role of AI in this loop has changed over the past decade. Early successes in AI for science came largely from specialized models that served as predictors or optimizers for well-defined scientific objects, such as protein structures, quantum wavefunctions, or molecular potentials~\citep{jumper2021alphafold,carleo2017solving}. More recently, language models have been treated as researchers that take part in these discovery loops themselves, generating candidate solutions, writing and revising the programs that implement them, and carrying a line of inquiry across many steps in response to evaluator feedback~\citep{boiko2023autonomous,gottweis2026accelerating,lu2026towards,novikov2025alphaevolve}. Despite differences in domains, models, and search heuristics, these systems share a common building block, a reliance on the discovery loop, the \emph{propose-evaluate-refine} loop that drives new discovery results~\citep{romera2024funsearch,georgiev2025mathexplore,shojaee2025llmsr,yuksekgonul2026learning}.

% and have shown promise in discovering impressive solutions


% \james{Instead of framing simply scaling evaluation (simple best of N also scales eval), frame it as *structured* scaling of evaluation. Emphasize that we allocate evaluations in a structured way motivated by human research communities. This structured approach lead to much more effective discoveries across diverse domains.}
% \haotian{The difference from existing AI co-scientist work can also be discussed here, and then introduce the structured scaling thing.}


% What these systems leave unexamined is how the loop itself should be scaled in a structured way, so that more evaluations yields better discoveries. This leads to the study of test-time \emph{evaluation-driven scaling}, the scaling process of the discover loop that is primarily driven by evaluation signals from empirical measurements, simulations, formal checks, or performance profiles.
% Different from standard model scaling that scales up parameters and training data~\citep{kaplan2020scaling,hoffmann2022training}, or classical test-time scaling that scales through longer reasoning traces or additional agent turns~\citep{snell2024scaling,wu2024inference,muennighoff-etal-2025-s1,zhu2025scalingagents,liu2025budgetaware,kim2025scienceagentsystems}, evaluation-driven scaling in human research community is bottom-up, decentralized, and complicated, and a larger number of loops does not automatically imply better results. We aim to uncover the underlying structure how the cycles can be scaled up and compound, similar to what drives research community to advance science. 
% % While powerful, this process is slow and often takes years or even decades to yield major breakthroughs. 
% Specifically we ask: 
% \begin{center}
% \emph{how can AI-driven discovery loops be scaled in a principled and structured way, so that scientific breakthroughs can be accelerated significantly?}
% \end{center}

Over the past decade, the role of AI in scientific discovery has changed significantly. Early successes in AI for science came largely from specialized models that served as predictors or optimizers for well-defined scientific objects, such as protein structures, quantum wavefunctions, or molecular potentials~\citep{jumper2021alphafold,carleo2017solving,pfau2020ab,wang2018deepmd,zeng2023deepmd}. More recently, language models have been treated as researchers, generating candidate solutions, writing and revising the programs that implement them, and carrying a line of inquiry across many steps in response to evaluator feedback~\citep{boiko2023autonomous,gottweis2026accelerating,lu2026towards,novikov2025alphaevolve}. For instance, recent systems build the loop around evolutionary search procedures, as exemplified by AlphaEvolve and related approaches~\citep{novikov2025alphaevolve,romera2024funsearch,openevolve_github,lange2025shinkaevolve}, or around tree search~\citep{aygun2026era}, while other works adapt the model through test-time reinforcement learning on a single problem~\citep{wang2025thetaevolve,yuksekgonul2026learning}. Despite differences in domains, models, and search heuristics, these systems share a common building block: the \emph{propose-evaluate-refine} discovery loop that drives new discovery results~\citep{romera2024funsearch,georgiev2025mathexplore,shojaee2025llmsr,yuksekgonul2026learning}.




\begin{figure}[!tp]
  \centering
  \includegraphics[width=0.98\linewidth]{sections/figures/main_paper/introduction.pdf}
  \caption{\textbf{Overview of \method.}
  \textbf{(a)} \method mirrors the scientific community's
  \emph{propose--evaluate--refine} cycle, allocating the evaluator-query
  budget $N=C\times L\times K$ across three dimensions: global width $C$
  (independent lines explored in parallel), refinement depth $L$ (carrying
  promising lines forward and refining them), and local sample size $K$
  (comparing several ideas before committing to the best).
  \textbf{(b)} We explore applications spanning 28 open-ended discovery tasks across
  quantum circuit compilation, astrodynamics trajectory design, AI
  foundations, scientific algorithms, and mathematical discovery.
  \textbf{(c)} Representative state-of-the-art discoveries across these
  domains, all from a single open-source model.
  \textbf{(d)} Trajectory-level post-training fine-tunes the generator on its own high-performing trajectories, crediting each attempt by the trajectory's final outcome rather than its immediate score. It improves trajectory scores on both training and held-out tasks and establishes a new state of the art of $1.144887$ on the held-out Sum--Difference Problem.}
  % \haotian{remove the distribution figure and make text slighly bigger.}}
  % \haotian{Remove things after the best-evolve and simply say repeat. Constructor -> constructor}}
  \label{fig:hero}
\end{figure}


% Indeed, scientific discovery rarely proceeds as a single act of reasoning. 
% Run in parallel by a community of researchers who propose candidate solutions, test them against the world, and use the feedback to guide the next attempt~\citep{langley1987scientific}, 
% scaling this loop is exactly how the human science community jointly move science forward.
More broadly, the human research community advances science collectively by \emph{scaling this loop} in a complex, decentralized manner: researchers around the world pursue candidate solutions in parallel, driven by different inspirations, test them against the current baselines, and use the resulting feedback to shape the next attempts~\citep{langley1987scientific}.
With LLMs taking the role of individual researchers in the loop, the entire scaling can be designed completely differently: an organized, structured way to drive scientific breakthroughs more efficiently and effectively.
We name this new scaling dimension \emph{evaluation-driven scaling}, because it is primarily driven by evaluation signals from empirical measurements, simulations, formal checks, or performance profiles, which later on become inspirations of next proposals. 
Different from standard model scaling that scales up parameters and training data~\citep{kaplan2020scaling,hoffmann2022training}, or classical test-time scaling that scales through longer reasoning traces or additional agent turns~\citep{snell2024scaling,wu2024inference,muennighoff-etal-2025-s1,zhu2025scalingagents,liu2025budgetaware,kim2025scienceagentsystems}, 
evaluation-driven scaling targets challenging, open-ended problems that fundamentally require explorations, and a larger number of loops does not automatically imply better results. 
While showing promise in making discoveries, existing systems leave unexamined how the loop itself should be organized in a structured way. This leads to a central question: 
% We aim to uncover the underlying structure of how the cycles can be scaled up and compound, similar to what drives the research community to advance science. 
% Specifically, we ask: 
\begin{center}
\emph{How can AI-driven discovery loops be scaled in a structured way to accelerate scientific breakthroughs?}
\end{center}

% evaluation-driven scaling in the human research community is bottom-up, decentralized\haowei{I feel like we need to justify this. In some countries and universities, it seems ``bottom-up'' and ``decentralized'' are not true. Sometimes research is actually planned top-down.}, and complex, and a larger number of loops does not automatically imply better results

% The scaling of discover loops is recognized as \emph{evaluation-driven scaling}, because it is primarily driven by evaluation signals from empirical measurements, simulations, formal checks, or performance profiles, which later on become inspirations of next proposals. \haowei{for this paragraph, I will be curious how eval-driven scaling is related to the previously mentioned propose-evaluate-refine loop and the relevant methods. This paragraph seems disconnected from the last paragraph.}\haotian{See if addressed.}



% Different from standard model scaling that scales up parameters and training data~\citep{kaplan2020scaling,hoffmann2022training}, or classical test-time scaling that scales through longer reasoning traces or additional agent turns~\citep{snell2024scaling,wu2024inference,muennighoff-etal-2025-s1,zhu2025scalingagents,liu2025budgetaware,kim2025scienceagentsystems}, evaluation-driven scaling in the human research community is bottom-up, decentralized\haowei{I feel like we need to justify this. In some countries and universities, it seems ``bottom-up'' and ``decentralized'' are not true. Sometimes research is actually planned top-down.}, and complex, and a larger number of loops does not automatically imply better results. While showing promise in making discoveries, existing systems leave unexamined how the loop itself should be scaled in a structured way, so that more evaluations yield better discoveries. We aim to uncover the underlying structure of how the cycles can be scaled up and compound, similar to what drives the research community to advance science. 
% Specifically, we ask: 
% \begin{center}
% \emph{how can AI-driven discovery loops be scaled in a principled and structured way, so that scientific breakthroughs can be accelerated significantly?}\haowei{prefer to be in one line?}
% \end{center}

This paper introduces \method (\textbf{Simple} \textbf{T}est-time \textbf{E}valuation-driven \textbf{S}caling), a framework for scaling AI-driven discovery by structuring how evaluator queries are allocated and how evaluated histories are grown, filtered, and reused. The central challenge is to determine how early attempts and their evaluation signals should guide later proposals, and which search structures allow progress to compound on open-ended problems. \method draws on structural features of scientific communities: locally, individual researchers test a few variants and carry forward the best; over time, researchers selectively learn from prior results based on relevance, performance, and reputation; collectively, researchers build on one another's ideas to refine and propose new solutions; and in parallel, multiple lines of inquiry develop and compete. \method operationalizes these features through a compact and structured design tuple $(C,L,K,\Phi)$. Global width $C$ maintains independent trajectories, refinement depth $L$ lets feedback accumulate within each trajectory, local sample size $K$ filters candidate variants before they shape future refinement, and the proposal constructor $\Phi$ selects and compresses useful prior solutions, failures, and feedback into the next prompt. This reframes discovery-loop scaling as a problem of managing evaluated histories, so that additional evaluations compound into stronger trajectories rather than merely producing more attempts. 
% A detailed comparison between \method and recent AI discovery systems, including AlphaEvolve, OpenEvolve, Google Co-Scientist, and related evaluation-driven search methods, is provided in Supplementary Section A.
The key distinction between \method and existing AI discovery systems such as AlphaEvolve lies in the focus. Existing systems typically seek to maximize discovery performance through customized agentic search procedures. \method instead asks how the discovery loop itself should be organized and scaled. By isolating this structure, \method becomes a simple, structured, and highly parallelizable system that scales efficiently to tens of thousands of evaluator queries, yielding better results using smaller open-source models compared to prior systems that used larger proprietary LLMs. 
% \haotian{Still vague to people}
% \rahul{The key distinction from existing AI discovery systems lies in the object of study: existing systems typically build around a particular evolutionary search procedure, often embedded within broader agentic machinery, to maximize discovery performance, while \method asks how the discovery loop itself should be organized and scaled. By isolating this structure, \method provides a simple, structured, and efficient way to scale the loop to tens of thousands of evaluator queries, yielding results beyond those reached by prior systems even when they are paired with substantially stronger LLMs.}
% \haotian{Unlike existing AI discovery systems that combine evaluator-guided search with method-specific machinery such as evolutionary archives, agentic controllers, model ensembles, or online model adaptation, \method isolates the structure of the discovery loop itself. It provides a simple, structured, and efficient way to scale tens of thousands of evaluator queries, yielding results beyond those reached by prior systems even when they are paired with substantially stronger LLMs.
% Unlike existing AI discovery methods that XXX, \method provides a simple, structured, and effective way to scale up discovery loops to tens of thousands efficiently, providing SOTA results that existing AI discovery systems with much stronger LLMs cannot. 
A comprehensive comparison can be found in Supplementary~\ref{sec:related:existing_tte}.



We apply \method on 28 open-ended problems across diverse scientific domains, spanning quantum circuit compilations, astrodynamics trajectory designs, GPU kernel implementation, LLM scaling law designs, biological and time-series algorithms optimization, and mathematical constructions.
On all problems, \method discovers the \emph{state-of-the-art} solutions using a single open-source GPT-OSS model, surpasses both human experts and other AI discovery systems that use an order of magnitude larger proprietary models.
% far larger proprietary\haowei{how to define ``large'' here? how to know the size of a proprietary system?}. These results come from a single framework and , an order of magnitude smaller than frontier models. 
% That one configuration reaches every result across these diverse domains, with only the problem specification and the evaluator changing between them, points to evaluation-driven scaling itself as the source of the gains. 
To illustrate, \method improves the best-known bound for the Erd\H{o}s minimum-overlap problem, open in extremal combinatorics since 1955, ahead of every prior human and machine record~\citep{novikov2025alphaevolve}. It discovers quantum compilation policies that reduce expensive qubit-swap gates by over 20\% relative to the widely used LightSABRE baseline~\citep{zou2024lightsabre}. It improves the fuel efficiency of Solar System exploration mission trajectories, reducing propulsive costs by up to 23\% relative to references constructed from historical encounter sequences under the same orbital-dynamics evaluator~\citep{vasile2006MGA-diffculty,shen2026deepspacetrajectorydesign}. It implements the fastest TriMul kernel, the triangle multiplicative update central to AlphaFold3~\citep{jumper2021highly,abramson2024alphafold3}, and a lasso path solver $2.17\times$ faster than the widely used \texttt{glmnet}~\citep{friedman2010regularization}. In neuroscience, it also discovers a state-of-the-art whole-brain neural-activity predictor, reducing error by $8.5\%$ on the long-horizon time-series forecasting task in ZAPBench~\citep{lueckmann2025zapbenchbenchmarkwholebrainactivity} relative to the proprietary-model-driven algorithm discovery result~\citep{aygun2026era}. More than any single record, what matters is that one unchanged procedure produces all of them, from abstract mathematical constructions to executable scientific programs, showing that \method can serve as a general mechanism for discovery. 
% \haotian{Maybe more diverse? like time series prediction or symbolic regression would help justify ``diverse'' in the title.}

The above results come from the fixed, off-the-shelf GPT-OSS model, which is not specifically optimized for the long-horizon discovery that \method performs: standard post-training tends to reward outputs that score well immediately, whereas discovery often turns on unconventional attempts that score poorly on their own yet lead to much stronger solutions. This raises a natural question: how can the LLM itself be deliberately trained for long-horizon discovery? We address this by post-training the model on its own successful trajectories, crediting each attempt by the final outcome of its trajectory rather than its immediate score. The improved model then drives the same search, now less myopic and more willing to build on early failures in pursuit of a stronger eventual solution. We study training primarily in mathematics, across a range of related open-ended problems. Post-training improves the entire outcome distribution, raising both the average score across independent trajectories and the best score on problems where the off-the-shelf GPT-OSS model scores poorly, and it transfers to held-out mathematical problems. These results suggest the trained model learns to search for strong eventual solutions rather than optimizing for immediate scores.

In summary, \method takes the scaling of the loop as its object of study, and asks how a fixed budget of evaluator queries should be structured. By formalizing this structured scaling with the design tuple $(C,L,K,\Phi)$, \method shows superior performance using the open-source model, surpassing existing systems that uses larger proprietary models.
% \haowei{actually I think systems and models can be decoupled. ``paired with'' will be better than ``rely on'' from my POV}. 
\method uses a single configuration to handle all five domains and discover 28 SOTA results, with only the evaluator changing between problems. 
A summary of \method result with the open-sourced model can be found in \Cref{tab:summary_28_problems}.
% Furthermore, post-training credits each attempt by the final outcome of its trajectory, matching the long-horizon nature of discovery.
% \haowei{(minor) I am not sure if this intro is too long.}

% \rahul{Here are some crude thoughts: \method departs from prior LLM-driven discovery systems in what it studies about the discovery loop. Systems such as FunSearch, AlphaEvolve, OpenEvolve, and ShinkaEvolve~\citep{romera2024funsearch,novikov2025alphaevolve,openevolve_github,lange2025shinkaevolve} build the loop around a specific evolutionary search procedure; ERA~\citep{aygun2026era} builds it around tree search; and ThetaEvolve and TTT-Discover~\citep{wang2025thetaevolve,yuksekgonul2026learning} adapt the model through test-time reinforcement learning on a single problem. In each the search loop is not itself dissected into components that can be scaled. \method instead takes the scaling of the loop as its object of study, and asks how a fixed budget of evaluator queries should be structured: how to divide it among independent exploration, refinement depth, and local selection, and how to construct each generation from past attempts. This structured scaling is captured by the compact design space $(C, L, K, \Phi)$, for which we give a P\'olya-urn analysis of why these axes are jointly necessary. The proposer is held to a single minimal language-model call, so that any gain is attributable to how the budget is allocated rather than to machinery inside the proposer. \method runs the same open model, \texttt{gpt-oss-120b}, as OpenEvolve~\citep{openevolve_github} and TTT-Discover~\citep{yuksekgonul2026learning}, so its gains over them trace to how the evaluation budget is structured and scaled across $(C, L, K, \Phi)$. Against AlphaEvolve~\citep{novikov2025alphaevolve} and ERA~\citep{aygun2026era}, which run on much larger proprietary models, that same small model stays competitive, indicating that discovery at this level does not depend on a larger or richer proposer. A single configuration handles all five domains, with only the evaluator changing between problems. Its additional post-training credits each attempt by the final outcome of its trajectory, matching the long-horizon nature of discovery; ThetaEvolve~\citep{wang2025thetaevolve} and TTT-Discover instead reward each attempt on its immediate score.  \method also differs in setting from autonomous ``AI co-scientist'' systems~\citep{gottweis2026accelerating,boiko2023autonomous}, which tackle problems without automatic evaluators and rely on a scientist in the loop to judge natural-language hypotheses.}

% \subsection*{Results}


\begin{table*}[!t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.2pt}
\renewcommand{\arraystretch}{1.02}
\caption{Summary of \method results across 28 discovery problems, all using the open-sourced \texttt{gpt-oss-120b} model. We include the best human results and recent AI-discovered results as of April 22$^{nd}$, 2026. Results obtained with the post-trained model, e.g., the SOTA score on the Sum-Difference problem (1.144887), can be found in \Cref{fig:math_final}.}
\label{tab:summary_28_problems}
\begin{tabular}{@{}
>{\raggedright\arraybackslash}p{0.110\textwidth}
>{\raggedright\arraybackslash}p{0.240\textwidth}
>{\raggedright\arraybackslash}p{0.150\textwidth}
>{\raggedright\arraybackslash}p{0.235\textwidth}
>{\centering\arraybackslash}p{0.082\textwidth}
>{\centering\arraybackslash}p{0.083\textwidth}@{}}

\toprule
\textbf{Domain}
& \textbf{Problem}
& \textbf{Metric}
& \textbf{Prev best method}
& \textbf{Prev best}
& \textbf{\method} \\
\midrule

\multirow[c]{2}{=}{Quantum compilation}
& Superconducting qubit routing
& Added SWAPs ($\downarrow$)
& LightSABRE~\citep{zou2024lightsabre}
& 20063
& \textbf{15147} \\

& Zoned neutral-atom compilation
& Execution time ($\downarrow$)
& ZAC~\citep{lin2025reuse}
& 29187.7
& \textbf{19507.5} \\
\midrule

\multirow[c]{5}{=}{Astrodynamics}
& Mariner~10
& Propulsive cost ($\downarrow$)
& Historical sequence~\citep{giberson_mariner_1975}
& 0.424147
& \textbf{0.326993} \\

& Voyager~2
& Propulsive cost ($\downarrow$)
& Historical sequence~\citep{kohlhase_voyager_1977}
& 3.503798
& \textbf{3.430214} \\

& Galileo
& Propulsive cost ($\downarrow$)
& Historical sequence~\citep{damario_galileo_1992}
& 0.823681
& \textbf{0.795108} \\

& Cassini
& Propulsive cost ($\downarrow$)
& Historical sequence~\citep{peralta_cassini_1995}
& 1.066682
& \textbf{0.820129} \\

& Rosetta
& Propulsive cost ($\downarrow$)
& Historical sequence~\citep{glassmeier_rosetta_2007}
& 1.736837
& \textbf{1.552968} \\

% Prospective Jupiter
% & Astrodynamics
% & Propulsive cost ($\downarrow$)
% & \rui{(no prescribed reference)}
% & \rui{N/A}
% & Feasible trajectory \\

\midrule

\multirow[c]{7}{=}{Scientific algorithms}
& Lasso regularization path
& Runtime in ms ($\downarrow$)
& \texttt{glmnet}~\citep{friedman2010regularization}
& 4139.4
& \textbf{2502.3} \\

& ZAPBench forecasting ($H=1$)
& Test MAE ($\downarrow$)
& ERA~\citep{aygun2026era}
& 0.0174
& \textbf{0.0165} \\

& ZAPBench forecasting ($H=4$)
& Test MAE ($\downarrow$)
& ERA~\citep{aygun2026era}
& 0.0221
& \textbf{0.0211} \\

& ZAPBench forecasting ($H=8$)
& Test MAE ($\downarrow$)
& ERA~\citep{aygun2026era}
& 0.0244
& \textbf{0.0230} \\

& ZAPBench forecasting ($H=16$)
& Test MAE ($\downarrow$)
& ERA~\citep{aygun2026era}
& 0.0267
& \textbf{0.0251} \\

& ZAPBench forecasting ($H=32$)
& Test MAE ($\downarrow$)
& ERA~\citep{aygun2026era}
& 0.0283
& \textbf{0.0259} \\

& Single-cell RNA-seq denoising
& Denoising score ($\uparrow$)
& TTT-Discover~\citep{yuksekgonul2026learning}
& 0.73
& \textbf{0.74} \\

\midrule

\multirow[c]{7}{=}{AI foundations}
& TriMul
& Runtime ($\downarrow$)
& Human expert~\citep{gpumode_trimul_leaderboard}
& 1.140
& \textbf{1.122} \\

& Asymmetric matrix multiplication
& Runtime ($\downarrow$)
& CUDA Agent~\citep{dai2026cudaagent}
& 0.747
& \textbf{0.440} \\

& Batched cumulative sum
& Runtime ($\downarrow$)
& NVIDIA CUB~\citep{nvidia_cccl_github}
& 0.147
& \textbf{0.104} \\

& Scaling law-parallel
& Extrapolation $R^2$ ($\uparrow$)
& SLDAgent (GPT-5)~\citep{lin2026sldagent}
& \textbf{1.000}
& \textbf{1.000} \\

& Scaling law-domain\_mix
& Extrapolation $R^2$ ($\uparrow$)
& SLDAgent (Gemini-2.5-Flash)~\citep{lin2026sldagent}
& \textbf{0.991}
& \textbf{0.991} \\

& Scaling law-lr\&bsz
& Extrapolation $R^2$ ($\uparrow$)
& SLDAgent (o4-mini)~\citep{lin2026sldagent}
& 0.611
& \textbf{0.712} \\

& Scaling law-u\_shape
& Extrapolation $R^2$ ($\uparrow$)
& Goose + GPT-5~\citep{lin2026sldagent}
& -0.232
& \textbf{-0.008} \\

\midrule

\multirow[c]{7}{=}{Mathematics discovery}
& Erd\H{o}s minimum overlap
& Overlap ($\downarrow$)
& Together AI~\citep{togetherai2026einsteinarena}
& 0.380871
& \textbf{0.380868} \\

% & First autocorrelation inequality
% & Bound ($\downarrow$)
% & Together AI~\citep{togetherai2026einsteinarena}
% & \textbf{1.502862}
% & 1.503871 \\

& Second autocorrelation inequality
& Bound ($\uparrow$)
& Together AI~\citep{togetherai2026einsteinarena}
& 0.961206
& \textbf{0.962694} \\

& Third autocorrelation inequality
& Bound ($\downarrow$)
& Together AI~\citep{togetherai2026einsteinarena}
& 1.454555
& \textbf{1.453675} \\

& Sum--Difference problem
& Ratio ($\uparrow$)
& AlphaEvolve V2~\citep{georgiev2025mathexplore}
& 1.121936
& \textbf{1.143975} \\
% & \textbf{1.144887} \\

& Circle packing ($n=26$)
& Sum of radii ($\uparrow$)
& AlphaEvolve V2~\citep{georgiev2025mathexplore}
& \textbf{2.635983}
& \textbf{2.635983} \\

& Circle packing ($n=32$)
& Sum of radii ($\uparrow$)
& AlphaEvolve V2~\citep{georgiev2025mathexplore}
& \textbf{2.939572}
& \textbf{2.939572} \\

& Hadamard determinant ($n=29$)
& Determinant ($\uparrow$)
& Orrick~\citep{orrick2003newlower}
& \textbf{0.935673}
& \textbf{0.935673} \\

\bottomrule
\end{tabular}
\end{table*}

\subsection*{Overview of \method}
\label{subsec:method}
 
\method is a test-time framework for scientific discovery on problems that have a \emph{verifiable evaluation protocol}, which we call an \emph{evaluator}. An evaluator is the system's interface to the scientific objective: given a candidate solution, it returns a numerical score together with auxiliary feedback such as verifier messages, error traces, or runtime statistics. Depending on the task, it may compute the objective exactly (an exact verifier), estimate it empirically (a measurement), or approximate it (a heuristic proxy). The objective is to find the highest-scoring candidate under the evaluator.
 
Formally, a problem is specified by an instruction $x_0$, and the goal is a solution $y$ that maximizes the score $r$ output by an evaluator $V$. To search for such a solution, an LLM $G$ plays the role of a researcher, drawing candidates $y \sim G(x)$ from a proposal $x$ built from the instruction $x_0$ together with the accumulated history of previously evaluated solutions, their scores, and the evaluator's feedback. \method runs this as a \emph{propose--evaluate--refine} loop: $G$ proposes a candidate, $V$ evaluates it, and its score and feedback are folded into the history that shapes the next proposal.
 
\method organizes this loop through a compact design tuple
\begin{align}
    (C, L, K, \Phi),
\end{align}
where $C$ is the number of parallel trajectories, $L$ the number of refinement steps per trajectory, $K$ the number of candidates drawn per step, and $\Phi$ the proposal constructor that assembles each new proposal from a trajectory's history. \method launches $C$ independent trajectories and advances each for $L$ refinement steps. At each step, $\Phi$ builds a proposal $x$ from the history so far, $G$ draws $K$ candidate solutions from $x$, $V$ scores them, and the highest-scoring one is appended to the trajectory. Once every trajectory has completed, \method returns the best solution across all of them, having spent $N = C \times L \times K$ evaluator queries.
 
This decomposition is what gives \method its structure: each of the three dimensions targets a distinct, independent way an undirected search fails, so together they form a small and non-redundant set of controls on the search, which we analyse and ablate in the Methods. Refinement depth $L$ lets feedback accumulate, so later attempts build on earlier ones, but a single deep trajectory is not enough, since once early attempts bias the search toward a narrow direction, further refinement tends to reinforce that basin rather than escape it. Global width $C$ counters this by running independent trajectories in parallel, so competing directions mature without influencing one another early on. Local sample size $K$ addresses noise in the LLM's output: drawing several candidates at each step and committing only the highest-scoring one keeps a weak or non-executable candidate from corrupting every later refinement built on it. Because the three act on different failure modes, they can be adjusted independently, and the budget $N$ has a clear meaning as the way that scaling is allocated.

In practice, the allocation of the evaluator-query budget across $C$, $L$, and $K$ depends on the task. Problems whose progress depends on discovering qualitatively different approaches, such as mathematical construction problems, benefit from larger $C$, whereas problems dominated by incremental engineering refinement, such as GPU kernel optimization, benefit from larger $L$. The local sample size $K$ should remain moderate: increasing it makes each committed step more reliable, but leaves fewer refinement steps under the same budget. Unless otherwise stated, we use $C=32$, $L=100$, and $K=16$ as a default configuration.
 
While $C$, $L$, and $K$ govern how evaluated histories grow, the proposal constructor $\Phi$ governs which parts of that history are reused, since a trajectory's history soon becomes too long and noisy to feed back in full. Because each proposal can build on several prior attempts rather than only the last, the history forms a directed graph rather than a chain. $\Phi$ selects which attempts to reuse through a graph-based variant of the PUCT rule~\citep{rosin2011multiarmed,silver2017mastering,alphazero2018}, favoring attempts that scored well or led to strong later attempts, while still giving promising but rarely used ones a chance to be revisited. It also folds in a running summary of recurring failures, such as compilation errors, verifier failures, or timeouts, to steer $G$ away from unproductive directions. 
% The full selection rule and its parameters are given in Methods.
In Methods, a Pólya-urn analysis together with ablations on $C$, $L$, and $K$ shows why these dimensions form a compact design space for scaling the loop, and $\Phi$'s construction and selection strategy are specified and ablated in full. We next turn to the discoveries \method makes across scientific domains, and then to how a language model can be trained for \method-based discovery. 


\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{sections/figures/main_paper/fig2_quantum_layout.pdf}
\caption{
\textbf{\method{} discovers quantum compilation policies across superconducting and zoned neutral-atom devices.}
\textbf{(a)}
Superconducting routing maps logical two-qubit gates onto sparse coupling graphs by choosing an initial layout and inserting SWAPs when needed. The evaluated coupling maps are \texttt{Q20}, \texttt{Willow}, and \texttt{Heron}~\citep{li2019tackling,google2025willow,nation2021heavyhex,ibm2026hardware}.
\textbf{(b)}
Across 72 superconducting routing cases on \texttt{Q20}, \texttt{Willow}, and \texttt{Heron}, SimpleTES lowers average added SWAP overhead by 21.7\% versus \textsc{SABRE} and 14.9\% versus \textsc{LightSABRE}; win/tie/loss counts are 56/10/6 and 38/13/21~\citep{li2019tackling,zou2024lightsabre}.
\textbf{(c)}
Representative \texttt{sym9\_193} case on \texttt{Q20}. Native CNOT gates are directly executable under the start layout. \textsc{LightSABRE} executes 24 CNOT gates with 16 inserted SWAPs, whereas SimpleTES selects a start layout where all 24 CNOTs are native and no SWAPs are needed.
\textbf{(d)}
Zoned neutral-atom routing maps logical stages to Storage and Entangling SLM placements, then loads and returns atoms with AOD batches. The examples illustrate order-preserving parallel transport and ghost-spot constraints~\citep{bluvstein2022quantum,bluvstein2024logical,stade2024abstract,lin2025reuse}.
\textbf{(e)}
On 36 neutral-atom benchmarks, SimpleTES total runtime normalized to the ZAC-style baseline is shown by circuit category. The overall geometric mean is 0.668, corresponding to a 33.2\% total execution time reduction~\citep{lin2025reuse,li2023qasmbench,quetschlich2023mqt}.
\textbf{(f)}
In the representative \texttt{dnn\_n8} case, SimpleTES keeps the active frontier on one entangling row, reducing stage 6 AOD routing from 4 rounds/12 commands to 2 rounds/6 commands. Full-plan execution time drops from 4.17 ms to 2.05 ms.
% a 50.7\% reduction.
}
\label{fig:quantum_compilation_six_panel}
\end{figure*}


\subsection*{\method{} discovers effective algorithms to reduce quantum compilation overhead}
\label{sec:task:quantum}



Quantum computing is an increasingly important computing paradigm that stores and processes information via quantum-mechanical systems~\citep{nielsen2010quantum}.
Whereas a classical bit has a definite value of either 0 or 1, a quantum bit, or \emph{qubit}, can be in a coherent superposition of both states.
By manipulating such states and creating correlations between qubits through entangling operations, quantum computers can obtain polynomial or exponential speedups for selected problem classes~\citep{shor1994algorithms,grover1996fast,farhi2014quantum,harrow2009quantum,biamonte2017quantum,feynman1982simulating,lloyd1996universal,aspuru2005simulated}.
At the center of this paradigm is the quantum algorithm, which specifies how quantum operations transform input states into desired outputs.
In the circuit model, a quantum algorithm is represented by a quantum circuit: an ordered sequence of elementary operations, called \emph{gates}, applied to logical qubits~\citep{nielsen2010quantum}.
One-qubit gates update the state of a single qubit, while two-qubit gates create interactions between a pair of qubits.
A logical circuit may specify two-qubit gates between arbitrary pairs of logical qubits, but a real device can apply a direct two-qubit gate only when the corresponding physical qubits satisfy the hardware's interaction constraints, thus creating a compilation problem of how to assign logical qubits to physical qubits and update that assignment over time so that every required two-qubit gate becomes executable. The additional operations introduced in this process are costly and error-prone, making overhead reduction the central optimization goal.



This optimization problem is computationally challenging and takes different forms on different hardware platforms~\citep{ito2023algorithmic,siraichi2018qubit,cowtan2019qubit,bluvstein2024logical,stade2024abstract,lin2025reuse,stade2025routing,tan2025compilation}. We use \method{} to address two representative hardware settings, superconducting platforms and neutral-atom architectures.
% Computational hardness is a central obstacle in the compilation problem we study, and it arises in different forms across the two representative hardware settings considered here (\Cref{fig:quantum_compilation_six_panel}a,d). 
In superconducting devices, physical qubits occupy fixed chip locations and allowed two-qubit interactions form a sparse coupling graph; compilation must choose an initial layout and insert SWAP gates when interacting logical qubits are mapped to non-adjacent physical qubits~\citep{li2019tackling,zou2024lightsabre}.
% , with the resulting routing problem being NP-hard~\citep{ito2023algorithmic,siraichi2018qubit,cowtan2019qubit,li2019tackling,zou2024lightsabre}. 
In zoned neutral-atom devices, atoms are kept in a storage zone or moved to an entangling zone for Rydberg gates; compilation must choose placement snapshots whose transitions can be realized through AOD-mediated movement.
% , and the resulting compilation pipeline involves subproblems with NP-hard formulations~\citep{bluvstein2024logical,stade2024abstract,lin2025reuse,stade2025routing,tan2025compilation}.
Together, these settings contrast fixed-graph routing with geometry-limited atom placement and rearrangement, while retaining the same high-level goal of minimizing extra hardware work.
We apply \method{} within fixed compilation scaffolds that isolate editable policy components, with necessary correctness checks applied.
For superconducting circuits, \method{} edits the initial layout and online SWAP selection rule; candidate routers are compared against \textsc{SABRE}~\citep{li2019tackling} and \textsc{LightSABRE}~\citep{zou2024lightsabre}, with added SWAP overhead as the cost.
For zoned neutral-atom compilation, \method{} edits only the placer in a fixed scheduler--reuse-analyzer--placer--router pipeline, with the remaining modules held fixed; candidate placers are compared against a reuse-aware ZAC-style baseline~\citep{lin2025reuse}, with total execution time as the objective.
Formal problem definitions, hardware constraints, and optimization objectives
for both compilation tasks are given in
Supplementary~\ref{app:quantum_problem_definition}.
Benchmark suites, baselines, and evaluation metrics are provided in
Supplementary~\ref{app:quantum_policy_details}.

Across both settings, \method{} achieves substantial overhead reductions relative to established baselines, driven by a shared design principle: place important logical qubits near useful hardware locations before expensive routing or rearrangement becomes unavoidable.
In superconducting routing, the best policy reduces topology-averaged added SWAP overhead by 21.7\% relative to \textsc{SABRE} and 14.9\% relative to \textsc{LightSABRE}, with the largest reductions on \texttt{Q20} reaching 33.3\% and 24.5\%, respectively; it implements the shared principle by mapping high-traffic logical qubits toward high-degree physical qubits, refining the assignment by local search, and scoring online SWAPs using a broader candidate neighborhood, look-ahead information, and immediate gate executability (\Cref{fig:quantum_compilation_six_panel}b,c).
In zoned neutral-atom compilation, the best placer discovered by \method{} reduces the geometric mean of total execution time by 33.2\% relative to the ZAC-style baseline; it implements the same principle through the sequence of placement snapshots passed to the fixed AOD router, preserving relative qubit order, reducing travel distance without losing AOD parallelism, and refining placements through reverse-time passes (\Cref{fig:quantum_compilation_six_panel}d--f).
Further details of the best discovered programs and the additional superconducting routing policy obtained using \method{} with Gemini are provided in Supplementary~\ref{app:quantum_discovered_programs} and \ref{app:superconducting_gemini}.




\subsection*{\method{} improves optimizers for fuel-efficient deep-space trajectories}
\label{sec:task:astrodynamics}


\begin{figure*}[p]
    \centering
    \includegraphics[width=0.98\linewidth]{sections/figures/main_paper/astrodynamics_task_compat.pdf}
    \caption{\textbf{Fuel-efficient deep-space mission design with evolved optimizers.} \textbf{(a)} Task abstraction and prospective Jupiter-window example. 
    \method searches over encounter sequences, maneuver placement, and continuous trajectory variables such as event times. 
    Gravity assists reshape the heliocentric trajectory without propellant expenditure, whereas DSMs add fuel cost. 
    In the 2028--2030 launch window, \method identifies an evaluator-feasible trajectory that reaches Jupiter in 2035 with \emph{no intermediate DSMs}.
    \textbf{(b)} Historical mission-window comparisons. 
    References are constructed from the corresponding historical encounter sequences and evaluated under the same simplified patched-conic model, constraints, and cost definition as \method{}, rather than using flown mission $\Delta v$ budgets. 
    The evolved optimizers find lower same-evaluator propulsive cost in all five windows.
    \textbf{(c)} Sources of improvement across the five historical benchmarks. 
    Timelines compare the encounter sequences and event times of each reference and best evolved trajectory; triangles mark DSMs of at least $10\,\mathrm{m\,s^{-1}}$. 
    For Galileo and Rosetta, the gains come from sequence optimization with continuous-variable optimization; The improvement of Mariner~10, Voyager~2, and Cassini is from continuous-variable optimization within independently recovered reference sequences.}
    \label{fig:astro_summary}
\end{figure*}


Deep-space missions often reach distant targets by using planets as moving gravitational waypoints rather than flying directly. 
A gravity assist (GA) uses a planetary flyby to reshape the spacecraft's heliocentric path with little propellant, whereas a deep-space maneuver (DSM) uses an engine burn to adjust the path~\citep{negri_historical_2020}. 
Designing such missions is difficult because route choices and timing choices are tightly coupled: the optimizer must choose which bodies to encounter, which transfer branches to use, and where maneuvers may be inserted, while also setting launch and encounter epochs and maneuver variables~\citep{vasile2006MGA-diffculty,shen2026deepspacetrajectorydesign}. 
We formulate this as an evaluation-driven discovery task in which each candidate produced by \method{} is an executable mission-design program. Given mission windows, a target body, allowed flyby bodies, and endpoint conditions, the program proposes complete multi-gravity-assist trajectories (\Cref{fig:astro_summary}a); an independent patched-conic evaluator reconstructs the trajectory from ephemerides~\citep{Folkner2014DEeph}, transfer arcs~\citep{izzo2015lambert}, flybys~\citep{minovitch1961method}, DSMs, and endpoint costs, rejects constraint violations, and scores feasible designs by verified propulsive cost.

We benchmark \method{} on five historical mission-window benchmarks and a prospective Jupiter exploration window. 
For the historical benchmarks, the comparison is not to flown mission $\Delta v$ budgets, which incorporate operational choices, navigation margins, and mission-specific high-fidelity modeling. 
Instead, each reference trajectory is constructed from the historical encounter sequence and nominal timing, then evaluated under the same orbital-dynamics model, feasibility constraints, and cost definition used to score \method{}. 
Across the historical mission windows, the best verified trajectories found by the discovered optimizers reduce propulsive cost in every case, by 2.1--23.1\% relative to these same-evaluator references (\Cref{fig:astro_summary}b). In the prospective 2028--2030 Jupiter exploration window, where no encounter sequence is prescribed, the discovered optimizer synthesizes an evaluator-feasible no-DSM Earth--Venus--Earth--Earth--Jupiter trajectory reaching Jupiter in 2035 (\Cref{fig:astro_summary}a).

Inspection of the evolved optimizers shows that the gains arise from reusable policies for coupled discrete--continuous mission design. 
The clearest sequence-level changes occur for Galileo and Rosetta (\Cref{fig:astro_summary}c): the Galileo optimizer finds Earth--Venus--Venus--Venus--Earth--Jupiter rather than the reference Earth--Venus--Earth--Earth--Jupiter sequence, while the Rosetta optimizer finds Earth--Earth--Earth--67P rather than Earth--Earth--Mars--Earth--Earth--67P. 
For Mariner~10, Voyager~2, and Cassini, the programs independently recover the reference encounter order and lower cost by refining the continuous trajectory variables within that sequence, showing that improvements do not require a different encounter sequence. 
Across cases, the evolved programs generate and prioritize candidate encounter sequences, allocate finite computation to promising time-of-flight regions, explore multiple transfer branches, combine global search with local refinement of encounter epochs and maneuver variables, and retain DSMs only when they reduce verified cost. 
Together, these results show that the evolved optimizers allocate finite computation both across encounter sequences and within each sequence's continuous design space.

% Inspection of the evolved optimizers shows that the gains arise from reusable search policies for mixed discrete--continuous mission design. 
% The discovered programs couple GA sequence construction with continuous trajectory refinement: they generate candidate encounter topologies from the mission specification, allocate search to promising time-of-flight regions, refine transfer arcs and encounter epochs, and insert DSMs only when the verified reduction in endpoint or correction cost outweighs the added burn. 
% This produces two qualitatively different modes of improvement.
% For Mariner 10, Voyager 2, and Cassini, the best trajectories independently recover the historical encounter order, while lowering the same-evaluator propulsive cost by improving timing and maneuver placement.
% For Galileo and Rosetta, \method{} changes the encounter topology itself, discovering lower-cost GA sequences under the same benchmark constraints; for example, the Galileo benchmark is improved by replacing the reference Earth--Venus--Earth--Earth--Jupiter sequence with an Earth--Venus--Venus--Venus--Earth--Jupiter sequence, while the Rosetta benchmark is improved by eliminating the Mars encounter and using an Earth--Earth--Earth--67P route (\Cref{fig:astro_summary}c). 
% In the prospective 2028--2030 Jupiter exploration window, where no encounter sequence is prescribed, the discovered optimizer synthesizes an evaluator-feasible Earth--Venus--Earth--Earth--Jupiter trajectory reaching Jupiter in 2037 with no intermediate DSMs (\Cref{fig:astro_summary}a). These results show that \method{} can evolve mission-design optimizers that search over both the planetary sequence and the continuous trajectory variables, rather than merely polishing a preselected historical route.


\subsection*{\method discovers better scientific algorithms}





Scientific algorithms are the computational methods that solve scientific problems: optimization solvers, forecasters, and learned models whose quality is judged by task-specific scientific objectives. These algorithms are usually produced by hand, often after years of accumulated domain expertise and engineering. We apply \method{} to three such problems and find that the same evaluation-driven search procedure discovers algorithms that improve over strong baselines: a geometry-aware lasso path solver that preserves strict correctness guarantees while outperforming the expert-engineered \texttt{glmnet} on real datasets; a whole-brain neural-activity forecaster that outperforms a prior proprietary-model search result; and a single-cell RNA-seq denoising algorithm that generalizes across datasets. We discuss the first two in detail below. Full denoising results are reported in the Supplementary Information, where an algorithm evolved exclusively on the Pancreas dataset matches the previous state of the art on held-out PBMC ($0.71$) and establishes a new best on held-out Tabula Muris Senis Lung ($0.74$ versus $0.73$) (Supplementary~\ref{app:denoising}).


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.98\textwidth]{sections/figures/main_paper/zapbench.pdf}
    \caption{\textbf{\method discovers a state-of-the-art whole-brain activity forecaster on ZAPBench.}
    \textbf{(a)} Neuronal activity forecast on a held-out frame: all $71{,}721$ neurons drawn at their anatomical centroids (dorsal $x$--$y$ projection) and colored by normalized activity ($\Delta F/F$), showing the ground truth, the \method prediction, and the absolute error on a shared scale.
    \textbf{(b)} Time series of  $2{,}000$ most active neurons from calcium recording under a single stimulus condition (\emph{turning}). Three subplots show the $4$-step window as the input of the prediction task, the
    prediction from \method within a $32$-step forecast window, and the absolute error compared to the ground truth within the same forecast window.
    \textbf{(c)} Per-condition held-out test MAE (mean $\pm$ s.d.\ over three seeds, averaged over the $32$-step horizon).
    \textbf{(d)} Held-out test MAE at $1$, $4$, $8$, $16$, and $32$ steps ahead, one panel per horizon on a shared $y$-axis (mean $\pm$ s.d.\ over three seeds; brown: ZAPBench baseline models \citep{lueckmann2025zapbenchbenchmarkwholebrainactivity}; teal: ERA \citep{aygun2026era}, an AI system that creates scientific software; deep teal: \method). The ERA and \method runs producing the 1-step forecasting results were optimized for the one-step prediction task only.
    \textbf{(e)} Test MAE versus prediction step ($1$ to $32$), pooled over all stimulus conditions and all neurons; the shaded band is $\pm 1$ s.d. across conditions.
    \textbf{(f)} The forecaster \method discovered: a shared-weight per-neuron network that predicts a residual from the last frame (identity skip) and blends it per-horizon with a linear-trend baseline, fed rich per-neuron features.}
    \label{fig:zapbench}
\end{figure}


% \haotian{Add lasso figure back here.}
\paragraph{\method discovers a geometry-aware lasso solver that surpasses \texttt{glmnet}.}
The lasso regularization path is a core computational primitive in high-dimensional statistics, used in cross-validation, model selection, and large-scale regression workflows from genomics to finance. The de facto solver, \texttt{glmnet}~\citep{friedman2010regularization}, encodes more than a decade of expert coordinate-descent engineering: warm starts, sequential strong-rule screening~\citep{tibshirani2012strong}, active-set inner loops, KKT verification, and a precision-matched switch between the covariance ($p < 500$) and naive residual ($p \geq 500$) updates. We ask whether evaluation-driven search, starting from a faithful C++ port of \texttt{glmnet} itself, can produce a strictly faster solver while preserving the same correctness guarantees. The evaluator is exact: candidate programs are self-contained C++ binaries, and a candidate is valid only if its per-$\lambda$ objective gap relative to \texttt{sklearn}'s solution stays below $10^{-6}$ on a held-out problem, with any failure forcing the score to zero. Evolution operates exclusively on synthetic problems, scored by the geometric mean of solve times across 17 procedurally generated instances that span sample-to-feature ratio, design-matrix sparsity, active-set density, and feature correlation. Because no real dataset is ever exposed to the search, the gains reported on real data below reflect generalization rather than tuning to the test set.

Across the 11 real-world datasets in Supplementary Table~\ref{tab:lasso_results}, none seen during the search, \method discovers a solver that is $2.17\times$ faster than \texttt{glmnet} on average and $14.08\times$ faster than \texttt{sklearn}, with every reported solution passing the held-out correctness check. What makes the discovered solver notable is not just raw speed but \emph{geometry awareness}: it reads the shape of each problem and adapts its algorithm accordingly. Where \texttt{glmnet} applies coordinate descent uniformly, \method's solver detects the problem regime and switches solver family to match it. For moderate-dimensional, tall designs ($p \leq 2000$ and $n \geq p/4$) it abandons coordinate descent for an exact LARS homotopy solver that traces the regularization path analytically, updating the active set at each kink with rank-one inverse Gram updates~\citep{efron2004least}; for wide or sparse designs ($p > 2000$ or $n < p/4$) it retains coordinate descent with strong-rule screening. This geometry-dependent switching is exactly what the speedups track: the gains peak at $9.56\times$ over \texttt{glmnet} on the tall DNA design ($1700 \times 180$, the only case with $n \gg p$), where the LARS branch fires on a small active set, settle at $1.30$--$1.50\times$ on wide biological designs where $p \gg n$, and reach $1.36$--$1.76\times$ on large mixed-shape datasets such as RCV1 and Gisette. The vs-\texttt{sklearn} gains are largest on the biological datasets, up to $50.77\times$ on TCGA BRCA. In effect, the discovered program recombines two well-known but historically separate lasso solver families into a single geometry-aware policy that selects the right one for each input, arrived at from no prior beyond the starting code and the evaluator. That the speedups hold on unseen real data suggests it exploits genuine problem structure rather than fitting the synthetic surrogate distribution.


\paragraph{\method discovers new state-of-the-art predictor for Zebrafish whole-brain neural-activity.}

Forecasting the neural activity of an entire vertebrate brain is a central challenge for understanding how brains turn sensory input and internal state into behavior~\citep{ahrens2013wholebrainimaging}. Continuous whole-brain recording at single-cell resolution is limited by motion artifact~\citep{Zong2022FreelyMovingMice}, photobleaching and phototoxicity~\citep{Laissue2017Phototoxicity}, and the trade-off between imaging speed and field-of-view~\citep{Prevedel2014LightField}. Predictive models bridge this gap by learning from recorded activity and stimulus context to forecast future brain states. The Zebrafish Activity Prediction Benchmark (ZAPBench)~\citep{lueckmann2025zapbenchbenchmarkwholebrainactivity}, built from a two-hour light-sheet recording of a larval zebrafish exposed to a sequence of visual stimuli, provides activity traces for $71{,}721$ neurons over $7{,}879$ time steps across nine stimulus conditions, with the task of predicting neural activities up to $32$ steps ahead from only $4$ steps of context. The strongest previously reported forecaster was discovered by Empirical Research Assistance (ERA)~\citep{aygun2026era}, a tree-search method guided by a proprietary frontier model; ERA and \method{} differ in both the search algorithm and the underlying model, and we ask whether \method{} with an open-sourced model can discover competitive forecasters on the same task under similar computational limits.

\method{} achieves the strongest forecasting performance on ZAPBench, outperforming prior methods at every evaluated horizon (\Cref{fig:zapbench}d): its horizon-averaged test MAE of $0.0259$ at 32 steps improves over ERA ($0.0283$; $8.5\%$ relative reduction) and the strongest ZAPBench baseline, the volumetric U-Net ($0.0292$; $11.3\%$ relative reduction). Its whole-brain prediction closely matches both the spatial organization and magnitude of the recorded population response (\Cref{fig:zapbench}a); the neuron-by-time raster preserves the dominant temporal structure of the recorded activity (\Cref{fig:zapbench}b). The prediction error varies across stimulus conditions (\Cref{fig:zapbench}c), and grows over the forecast horizon (\Cref{fig:zapbench}e).
The discovered program (\Cref{fig:zapbench}f) shows that \method{} improves performance by automatically identifying a compact, well-matched combination of forecasting modules and their parameterization. %\rahul{This is honest, but it slightly undercuts the "discovery" framing: if the win comes from combining known parts (residual/skip, NLinear normalization, linear-trend baseline, PCA features), a reviewer may ask whether this is discovery or engineering of standard components. the value is automatically finding the right COMBINATION and parameterization, rather than let it read as "nothing new"?}
The decisive change is to reformulate the prediction target: rather than regressing absolute future activity, the network predicts a residual added back through an identity skip connection, echoing residual learning~\citep{he2016deep} and last-value normalization from NLinear-style models~\citep{zeng2023dlinear}. Around this residual predictor it adds an explicit linear-trend baseline, combines it with the nonlinear forecasts using per-horizon closed-form least-squares weights, and feeds the nonlinear predictor a rich per-neuron descriptor including first-order differences, window slopes, per-step population statistics, and data-driven identity features from each neuron's low-rank SVD loadings and coupling to the brain-wide mean.




\subsection*{\method improves AI foundations}


\begin{figure}[p]
    \centering
    \includegraphics[width=\linewidth]{sections/figures/main_paper/AIfoundation_compat.pdf}
    \caption{Better AI foundations discovered across GPU kernel optimization and scaling-law extrapolation. (a) GPU kernel optimization task, where the optimizer translates a high-level operator into an architecture-aware implementation and minimizes execution time on a target GPU. (b) Discovered TriMul implementation with mixed precision, fused kernels, hierarchical tiling, and memory/thread mapping. (c) Kernel speedup comparisons for trimul, asymmetric matmul, and cumsum. (d) Scaling-law prediction task, where the optimizer converts small-scale training measurements into an extrapolative symbolic law and minimizes prediction error on larger target compute scales. (e) Discovered law predicts the target-scale LR \& BSZ loss landscape and selects near-optimal hyperparameters. (f) SLDBench results across models and frameworks, where higher accuracy indicates better performance.}
    \label{fig:ai_for_ai}
\end{figure}

Two important foundations of modern AI development are building efficient GPU kernels that make models run fast on real hardware (\Cref{fig:ai_for_ai}a), and discovering scaling laws that help predict how model performance changes as training is scaled up (\Cref{fig:ai_for_ai}d). Both have traditionally relied on expert manual design: GPU kernels are carefully optimized by systems engineers for specific hardware architectures and software stacks, while scaling laws are manually specified and fitted by researchers to predict how performance changes with model size, data size, compute, and other scaling variables. We apply \method to both classes of problem and find that the same evaluation-driven search procedure produces kernels that surpass expert Triton submissions and AI kernel-discovery baselines on real hardware, and scaling laws that extrapolate substantially better than the strongest agent baselines on the SLDBench benchmark.
 
\paragraph{GPU kernel optimization.}
We apply \method to optimize the GPU kernels that modern AI systems rely on. \method starts from a simple PyTorch reference implementation and searches for a faster GPU kernel that preserves numerical correctness within a task-specific tolerance. We evaluate this ability on three representative operators. The first is TriMul, a triangular multiplicative update used in AlphaFold3-class protein-structure models~\citep{abramson2024alphafold3,byte2025protenix} and the subject of an active GPUMode optimization competition~\citep{gpumode_trimul_leaderboard}. The second is asymmetric matrix multiplication, an irregular-shape GEMM pattern in modern AI workloads, including small-batch inference, LoRA adapters, and query-similarity search. The third is batched cumulative sum, a primitive in LLM sampling and stream-compaction pipelines. Across all three tasks, \method discovers kernels on an NVIDIA H200, and the resulting implementations are evaluated without re-tuning on the target GPUs. We compare against both expert-engineered kernels and recent AI-driven kernel-discovery systems baselines that achieve previous SOTA efficiency~\citep{yuksekgonul2026learning,cao2026ksearch,bicker2026aster,dai2026cudaagent}.

%On TriMul, \method produces the fastest Triton kernel reported to date on H100 (1.122~ms), surpassing the strongest human Triton submission on the GPUMode leaderboard (1.140~ms) and AI baselines (1.154--1.212~ms). The kernel, evolved on H200, also achieves the fastest runtime when transferred without re-tuning to NVIDIA A100, H100, and AMD MI300 (Supplementary Information \rahul{Needs reference. Make sure to include content on appendix and include reference here.}), indicating that the discovered implementation captures structure that generalizes across architectures. 

On TriMul, a kernel discovered by \method on H200 transfers directly to H100 without re-tuning, reaching a geometric-mean latency of 1.122 ms, surpassing both the AI baseline of 1.154 ms in~\Cref{fig:ai_for_ai}c and the strongest expert-written Triton baseline of 1.140 ms on the GPUMode leaderboard (Supplementary~\Cref{tab:app.trimul_align}). The same implementation achieves the fastest runtime on NVIDIA A100, NVIDIA H100, and AMD MI300, suggesting that the search found a portable implementation strategy rather than an H200-specific optimization (Supplementary~\Cref{tab:app.trimul_cross_hardware}). Inspection of the discovered implementation shows that the gain comes from jointly optimizing high-level structure and low-level kernel tuning. \method fuses layer normalization, gating, projection, and masking into a small number of Triton kernels, selects a mixed-precision path in which activations move in FP16 while reductions remain in FP32, and tunes tile sizes within the kernels to improve hardware utilization (\Cref{fig:ai_for_ai}b). The asymmetric-matmul and batched-cumsum tasks further show that \method can specialize the implementation strategy to the input shape, rather than relying on a one-size-fits-all template for each operator. On asymmetric matrix multiplication, the largest gains occur on highly uneven matrix shapes, where \method achieves up to $4.01\times$ speedup over the PyTorch FP32 reference and reduces runtime by 65.6\% relative to CUDA Agent on the case with the largest improvement (\Cref{fig:ai_for_ai}c). Batched cumulative sum provides a clearer example of shape-dependent implementation: the discovered kernel selects between single-tile and multi-tile execution paths according to workload size. This implementation outperforms NVIDIA's hand-tuned CUB \texttt{DeviceSegmentedScan} on four of the six evaluated shapes and reaches $6.06\times$ speedup over the PyTorch reference. CUB remains only marginally faster on the two smallest shapes, where its fixed segmented-scan strategy is already well matched to the input. These case studies show that \method can automatically discover optimization strategies that are typically hand-engineered in optimized GPU libraries. Detailed shape definitions are provided in the Supplementary~\Cref{tab:app.trimul-shapes,tab:app.asymmetric-matmul-shapes,tab:app.batched-cumsum-shapes}.



 
\paragraph{Scaling-law discovery.}
We evaluate \method on four tasks from the SLDBench benchmark~\citep{lin2026sldagent,lin2024selecting}, covering parallel scaling~\citep{chen2025parallel}, domain-mixture scaling~\citep{ye2024data}, learning-rate/batch-size co-scaling~\citep{li2025predictable}, and U-shape compute scaling~\citep{wu2024u}. The task is to discover a symbolic law $f_\theta$ together with a per-setting fitting procedure that extrapolates accurately to held-out larger-scale configurations, where each configuration specifies the scale variables and task-specific control variables used for fitting and evaluation. Success is measured by the extrapolation coefficient of determination ($R^2$) on each task's extrapolation split. To isolate the effect of the search strategy, we use the same initialization, task instructions, and evaluator as the SLDAgent baseline~\citep{lin2026sldagent}: the initial program is a naive power-law function paired with a BFGS optimizer. Across the four tasks (\Cref{fig:ai_for_ai}d, Supplementary~\Cref{tab:sldbench_combined_with_simpleevolve}), \method achieves the best average $R^2$ of 0.674, exceeding the strongest baseline (SLDAgent with GPT-5, 0.572) and every other configuration tested. The advantage is sharpest on the hardest extrapolative settings: \method achieves the highest $R^2$ on the U-shape compute-scaling task (\texttt{u\_shape}; $-0.008$, versus $-0.232$ for the next-best baseline) and on the learning-rate/batch-size co-scaling task (\texttt{lr\&bsz}; 0.712 versus 0.611 for SLDAgent+o4-mini), where most agents obtain negative test-set $R^2$ and fail to extrapolate. The discovered law on \texttt{lr\&bsz} produces a hyperparameter recommendation only 0.058\% above the true optimum at a 1B-parameter, 100B-token target setting, corresponding to a 10$\times$ extrapolation in model size and a 100$\times$ extrapolation in data size (Supplementary~\ref{app.sld}).

 
These two task families share an interface---an initial solution and a queryable evaluator---and differ only in what the evaluator measures (wall-clock runtime under a correctness tolerance for kernels; held-out extrapolation $R^2$ for scaling laws). What unites them substantively is that both produce artifacts that AI development itself depends on: faster kernels reduce the cost of training and serving every downstream model, and more accurate scaling laws improve the decisions made before training begins. The same evaluation-driven scaling principle that surpasses expert Triton kernels on a competition leaderboard also discovers symbolic loss laws that extrapolate where strong agent baselines do not.


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{sections/figures/main_paper/math_composite_full.pdf}
%     \caption{\textbf{\method gains from post-training on generated trajectories.}
%       \textbf{(a--d)} Training-free results. Without any model training, \method reaches the best reported value on four classical problems, shown against prior human and AI records: \textbf{(a)} the Erd\H{o}s minimum-overlap problem ($0.380868$), with the discovered near-binary witness $h$; \textbf{(b)} the Second Autocorrelation Inequality ($0.962694$), with a sparse near-impulse witness; \textbf{(c)} the Third Autocorrelation Inequality ($1.453675$), with an oscillatory signed witness; and \textbf{(d)} the sum-difference ratio ($1.143975$), whose set has an arithmetic-progression backbone, illustrated by the $A$, $A{+}A$, $A{-}A$ schematic.
%       \textbf{(e--l)} Training results, with in-distribution tasks in the top row and held-out tasks in the bottom row; grey denotes the training-free model and blue the post-trained model.
%       \textbf{(e, i)} Average top-$R\%$ trajectory score at $R \in \{10, 25, 50, 75\}$ before and after post-training.
%       \textbf{(f, j)} The same top-$R\%$ scores across post-training iterations (TF, 2, 4, 6).
%       \textbf{(g, h, k, l)} Trajectory-score distributions before and after post-training for representative tasks, dashed lines marking the means: \textbf{(g)} AC2 and \textbf{(h)} a second in-distribution task in distribution; \textbf{(k)} circle packing $n{=}32$ and \textbf{(l)} the sum-difference ratio held out, where the post-trained model reaches $1.144887$.
%       Full per-task results are reported in the Supplementary~\Cref{fig:math_discovered_solutions,app:math_extremal_analysis,app:math_combinatorial_construction}.}
%     \label{fig:math_final}
% \end{figure}


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{sections/figures/main_paper/math_composite_full_compat.pdf}
    \vspace{-20pt}
    \caption{\textbf{\method gains from trajectory-level post-training.}
      \textbf{(a--d)} SOTA mathematics constructions that \method achieve with the open-sourced GPT-OSS model. Without model training, we surpass the best reported values on four classical problems: \textbf{(a)} the Erd\H{o}s Minimum-Overlap Problem ($0.380868$); \textbf{(b)} the Second Autocorrelation Inequality ($0.962694$); \textbf{(c)} the Third Autocorrelation Inequality ($1.453675$); and \textbf{(d)} the Sum--Difference Problem ($1.143975$), and reach the same optimum on the other three (Supplementary~\ref{app:math_extremal_analysis}, \ref{app:math_combinatorial_construction} and \Cref{fig:math_discovered_solutions}).
      \textbf{(e--l)} \method performance using the post-trained GPT-OSS model on four trained tasks (the top row) and four held-out tasks (the bottom row). The grey curve represents results obtained from the untrained model, and blue curve from the trained model.
      Panel \textbf{(e, i)} show the average top-$R\%$ trajectory scores for $R \in \{10, 25, 50, 75\}$ before and after post-training, panel \textbf{(f, j)} show the scores under different training iterations (TF: untrained, 2, 4, 6).
      Panel \textbf{(g, h, k, l)} show the score distributions for representative tasks, with dashed lines indicating the average scores across trajectories and dots along the bottom indicating individual trajectory scores. Notice that panel \textbf{(l)} corresponds to the held-out Sum--Difference Problem, on which the post-trained model reaches a new SOTA score $1.144887$.}
    \label{fig:math_final}
\end{figure}



\subsection*{Post-training the LLM for \method leads to new mathematical discoveries}
\label{subsec:mathematics}

To understand how post-training improves \method, we study eight mathematical problems spanning harmonic analysis, additive combinatorics, discrete geometry, and extremal matrix theory (Supplementary~\ref{app:math_tasks}), using four for training and holding out the other four for testing. We choose mathematical discovery as the testbed because each problem is can be scored by a deterministic evaluator, so an improvement is a verified bound rather than a noisy estimate. Without any model training, \method establishes new state-of-the-art constructions on four of the eight problems. On the Erd\H{o}s minimum-overlap problem, it lowers the objective from the previous best of $0.380871$, reported by Together AI~\citep{togetherai2026einsteinarena}, to $0.380868$. It also raises the Second Autocorrelation Inequality bound from the previous best of $0.961206$ to $0.962694$ and lowers the Third Autocorrelation Inequality bound from $1.454555$ to $1.453675$, improving upon two additional Together AI records~\citep{togetherai2026einsteinarena}. On the Sum--Difference Problem, it raises the previous best ratio of $1.121936$, established by AlphaEvolve V2~\citep{georgiev2025mathexplore}, to $1.143975$. \method also matches the existing records on three of the remaining problems (\Cref{fig:math_final}a--d). These results come entirely from search at test time, which raises a natural question: can the trajectories a run produces be folded back into the model, so that what the search discovers becomes part of its own capability?

We post-train the LLM on the trajectories the search itself produces. Rather than credit each attempt by its own evaluator score, which would reward only immediate gains, we credit every attempt in a trajectory by that trajectory's final outcome, the best score it eventually reaches. For each task we keep the trajectories whose outcome falls in the top $R\%$, set their weight $w{=}1$ and all others $w{=}0$, and fine-tune the LLM $\pi_\theta$ under the weighted likelihood
\begin{equation}
\label{eq:loss_main}
\mathcal{L} = -\,\mathbb{E}_{(x, \hat{y}, w) \sim \mathcal{D}}\!\left[ w \cdot \sum_{i=1}^{|\hat{y}|} \log \pi_\theta\!\left(\hat{y}_i \mid x, \hat{y}_{<i}\right) \right],
\end{equation}
where $x$ is the proposal context and $\hat{y}$ the model's reasoning and solution. We repeat this over several rounds, so that each round of post-training improves the LLM that produces the next round's trajectories. The full credit-assignment scheme and training procedure are described in the Methods, with hyperparameters and compute in Supplementary~\ref{sec:analysis_train}.

Because open-ended discovery aims to push the frontier rather than raise the mean, we evaluate by the average score of the top-$R\%$ of trajectories at $R\in\{10, 25, 50, 75\}$, which exposes how the upper tail of the distribution shifts after training. On the four training tasks, post-training moves the upper tail upward at every level (\Cref{fig:math_final}e,g); on the Erd\H{o}s problem the shift is large enough that the trained model's top-$25/50/75\%$ scores match the untrained model's top-$10/25/50\%$, and it accumulates over iterations rather than saturating after the first (\Cref{fig:math_final}f). The four held-out tasks show the same effect, with the upper tail lifted across levels (\Cref{fig:math_final}i) and gains that appear early and persist (\Cref{fig:math_final}j), indicating that post-training instills a discovery skill that generalizes beyond the trained tasks. Post-training also reaches a solution the training-free search does not find under the same budget: on the held-out sum-difference problem it improves the ratio from the training-free record of $1.143975$ to a new best of $1.144887$ (\Cref{fig:math_final}l). Post-training on a model's own successful trajectories therefore does more than lift the distribution in aggregate; it surfaces solutions beyond the reach of the untrained search.



% \subsection*{Discussion}
% \textcolor{red}{Not ready.}

% \haotian{Why figure number is reset in this section?}
% \textcolor{red}{What does you want to say in discussion and in each paragraph?
% \begin{enumerate}
%     \item Ablation of methods should be in the extended method not in discussion.
%     \item start with a summarized paragraph with additional information about \method.
%     \item difference about multi-agent system. MAS is a multiple calls having LLM calls and preserving it. We want to study the concept. 
%     \item Related works?
%     \item Reward hacking and limitations.
%     \item Efficiency, pruning, stronger model compatibility.
%     \item Future way of expanding the work?
% \end{enumerate}
% }

% \textcolor{red}{We need to clearly explain what has been captured from the science community, and what this C,L,K,$\Phi$ stands for, instead of giving readers possibility to challenge things like cross pollination, MAS, collaboration.}

% \haotian{I don't see what additional information you want to provide here. Seems like a very vague summary to me.}


\subsection*{Discussion}

\method reframes open-ended scientific discovery as a problem of structured scaling: how evaluator queries should be distributed across competing lines of inquiry, and how the resulting experience should guide subsequent attempts. Its design tuple $(C,L,K,\Phi)$ organizes this process across independent exploration, iterative refinement, local selection, and the selective reuse of evaluated history. Applying this same procedure and a single open model to 28 open-ended problems across five domains, while changing only the evaluator, \method reaches new state-of-the-art solutions across objectives ranging from exact mathematical verification and physical simulation to held-out prediction error and empirical hardware timing. More important than any individual record, these results show that evaluator queries become substantially more powerful when they are structured so that exploration and refinement can compound. Together, they establish structured evaluation-driven scaling as a general mechanism for discovery.

An important feature of these results is what \method deliberately holds fixed. For the cross-domain results above, each proposal is produced by a single call to the same LLM, without multi-agent coordination, multi-step agentic planning, model ensembles, or online parameter updates. In contrast, some existing discovery systems tend to combine evaluator-guided search with one or more of these components~\citep{novikov2025alphaevolve,openevolve_github,lange2025shinkaevolve,wang2025thetaevolve,yuksekgonul2026learning}, making it difficult to isolate the contribution of evaluation-driven scaling itself. By keeping the proposer minimal and making the allocation of evaluator queries explicit, \method shows that structured scaling is independently powerful: a single open model can match or surpass systems built around substantially more complex machinery. This does not imply that stronger models or more capable agents would provide no additional benefit; either could be incorporated into the same framework. Rather, the results establish that such complexity is not a prerequisite for discovery at this level and that the organization of the evaluation loop is itself an important source of capability.

The same structure also creates practical routes for scaling the discovery loop more efficiently. The $C$ trajectories can proceed independently, while the $K$ candidates conditioned on the same proposal can be produced in a single batched LLM request, exposing substantial parallelism and avoiding repeated processing of shared context. For instance, under matched evaluator-query budgets and runtime concurrency, \method reaches OpenEvolve's whole-run best score with an $11.8\times$ time-to-solution speedup on the third autocorrelation inequality problem, and an $18.0\times$ speedup on the sum-difference problem (Supplementary~\Cref{fig:app.efficiency}). The independence of trajectories also permits early pruning where trajectories can be stopped early on if they are not promising. For instance, under the most aggressive setting that retains only one trajectory after 25\% refinement steps, the trajectory that ultimately produced the best solution survives in 55\% problems, while relative score degradation remains below $0.01\%$ in most configurations and below $0.03\%$ in all configurations (Supplementary~\Cref{fig:pruning_dynamics}). This behavior is task-dependent, with pruning nearly lossless on circle-packing tasks but less reliable on the autocorrelation and Erd\H{o}s problems, where early scores are weaker indicators of eventual trajectory quality (Supplementary~\Cref{tab:pruning_strategies}). These results motivate adaptive allocation policies that redirect evaluator queries using not only intermediate scores but also trajectory growth and semantic signals.

% The trajectories collected by \method also provide a source of supervision for improving the LLM itself. Step-level optimization rewards each proposal according to its immediate score, but long-horizon discovery may depend on initially weak attempts that expose failure modes, introduce new directions, or provide useful foundations for later refinement. We therefore post-train the model on its own successful trajectories, assigning each attempt credit according to the best solution eventually reached by its trajectory rather than its immediate performance. Across four mathematical training tasks, this trajectory-level objective shifts the upper tail of the outcome distribution toward stronger solutions, and these gains transfer to four held-out problems (\Cref{fig:math_final}; Supplementary~\Cref{tab:irft_results,fig:irft_iteration}). On the held-out sum-difference problem, the post-trained model further improves the previous \method result from $1.143975$ to a new state-of-the-art value of $1.144887$. These findings suggest that the experience accumulated through structured evaluation-driven scaling can be internalized as search strategies that transfer beyond the problems used for post-training.

The power of evaluation-driven scaling also makes evaluator fidelity a central concern. Because \method optimizes the evaluator's score directly, it cannot inherently distinguish a genuine improvement in the intended objective from an implementation loophole that produces a higher score. Such exploits emerge even without access to the evaluator's source code. In mathematical construction tasks, the model exploits numerical tolerances, for example by producing circle packings with overlaps that fall just below the rejection threshold; in GPU-kernel optimization, it discovers more direct exploits, including caching outputs across timed runs, manipulating timing measurements, and corrupting the reference baseline (Supplementary~\ref{sec:method_analysis:reward_hacking_plenomena}). We address these failures by independently re-verifying reported results and manually hardening evaluators as new vulnerabilities appear. This preserves the validity of our reported discoveries, but the process is reactive: each patch invites the next exploit, and this approach will not scale to objectives that cannot be checked cheaply. A durable solution is to make the evaluator itself part of what is optimized, learning or co-evolving it alongside the search so that the surrogate remains aligned with the true objective.

Even with robust evaluators, the present framework remains limited to problems for which feedback can be obtained automatically and inexpensively enough to support repeated queries. Many important scientific objectives fall outside this setting because their evaluation is subjective, experimentally costly, or available only through slow physical or wet-lab measurements. In addition, the evaluator-query budget is divided across $C$, $L$, and $K$ using fixed values, although our analyses show that the most effective allocation depends on both the task and the evolving state of the search. \method also relies primarily on continuous, fine-grained scores to guide refinement, making it less naturally suited to problems with sparse or binary feedback, such as formal theorem proving, where near-misses and unproductive attempts may receive indistinguishable scores. Extending evaluation-driven scaling to these settings will require adaptive allocation policies, richer semantic feedback extracted from failed attempts, partial proofs, and textual critiques, and interfaces to higher-fidelity simulators, laboratory robotics, or real-world measurements. Together, these advances could enable discovery loops that allocate effort dynamically and learn from heterogeneous forms of scientific feedback while preserving reliable verification.


\subsection*{Code availability}

The complete SimpleTES codebase, which includes the evaluation-driven search framework, task definitions, evaluators, benchmark assets, released best-result artifacts, and analysis scripts, is publicly available at \url{https://github.com/wq-will/SimpleTES}, providing a transparent and extensible resource for reproducing, inspecting, and building on the experiments reported here.


\endgroup

